Area-Invariant Pedal-Like Curves Derived from the Ellipse

We study six pedal-like curves associated with the ellipse which are area-invariant for pedal points lying on one of two shapes: (i) a circle concentric with the ellipse, or (ii) the ellipse boundary itself. Case (i) is a corollary to properties of the Curvature Centroid (Kr\"ummungs-Schwerpunkt) of a curve, proved by Steiner in 1825. For case (ii) we prove area invariance algebraically. Explicit expressions for all invariant areas are also provided.

==> 065_videos.tex <==
Table~\ref{tab:videos} contains links to videos which illustrate some of the above phenomena. Column ``PL\#'' provides an index within a Youtube playlist.

\begin{table}[H]
\scriptsize
\begin{tabular}{|c|l|l|l|}
\hline
\href{youtu.be}{PL\#} & Title & Narrated \\
\hline
\href{youtu.be}{01} & 
\makecell[lt]{xxx} & no \\
\hline
\end{tabular}
\caption{Playlist of videos. Column ``PL\#'' indicates the entry within the playlist.}
\label{tab:videos}
\end{table}
